Canonical self-affine tilings by iterated function systems

An iterated function system $\Phi$ consisting of contractive similarity mappings has a unique attractor $F \subseteq \mathbb{R}^d$ which is invariant under the action of the system, as was shown by Hutchinson [Hut]. This paper shows how the action of the function system naturally produces a tiling $\mathcal{T}$ of the convex hull of the attractor. More precisely, it tiles the complement of the attractor within its convex hull. These tiles form a collection of sets whose geometry is typically much simpler than that of $F$, yet retains key information about both $F$ and $\Phi$. In particular, the tiles encode all the scaling data of $\Phi$. We give the construction, along with some examples and applications. The tiling $\mathcal{T}$ is the foundation for the higher-dimensional extension of the theory of \emph{complex dimensions} which was developed for the case $d=1$ in ``Fractal Geometry, Complex Dimensions, and Zeros of Zeta Functions,'' by Michel L. Lapidus and Machiel van Frankenhuijsen.

==> zeta-function.tex <==
\section{Building the geometry out of the scaling.}
\label{sec:zeta}

We are motivated in this section by the tube formula given in
\cite[Thm.~6.1]{FGNT}, and the relationships outlined in
\cite[Chap.~4.1.1]{FGNT} between the measure \gh and the geometric
zeta \fn $\gz_\gh$. Eventually,
%In particular, we will make use of
%the measure $\gh$ which is the \distl \deriv of $N_\L$ in
%\eqref{def:1-dim geom counting function}, and
we expect the tube formula for a self-similar tiling to be given
by a \distl expression of the form
\begin{equation}
  \label{eqn:V is eta on v}
  V(\ge) = \la \gh, v_\ge \ra,
\end{equation}
where $V(\ge)$ is the volume of the region within \ge of the
boundary of the tiling, as discussed in Def.~\ref{def:tube
formula}.

\gh is a local positive measure with support bounded away from 0
(i.e., a \emph{fractal string} in language of
\cite[Chap.~3.1]{FGNT}), which defines the density of geometric
states of the system. In other words, \gh encodes the \dist of the
scaled copies of the generators. For example, a point mass of
weight 2 above $x=3$ indicates that the inradius $\gr=1/3$ occurs
twice; this is discussed further in Def.~\ref{def:geom measure}
below.

$v_\ge$ is a polynomial which encodes geometric measure data for
the $k$-skeletons ($k=0,1,\dots,d$) of each generator $\gen_q$.
Thus, $v_\ge(x)$ gives the volume contribution of state $x$ to the
total inner tube volume $V(\ge)$.

In light of this interpretation of \gh and $v_\ge$,  \eqref{eqn:V
is eta on v} is just a \distl version of the basic notion
\begin{equation}
  \label{eqn:basic idea}
  \text{Total value}
  = \sum (\text{value of an }x) \times (\text{number of }x\text{'s})
\end{equation}
where the sum is taken over all different types of items $x$.

Once the concept behind this formula is clear, we can define \gzh
directly from \gh via the reciprocity described in
\cite[Def.~3.1]{FGNT} and \cite[Chap.~4.1.1]{FGNT}:
\begin{align}
  \label{eqn:density of states}
  \gh(x) %&= \int_0^\iy \gd_y(x) \, \gh(dy) \notag \\
         %&= \int_0^\iy \frac1{2\gp i} \int_{c-i\iy}^{c+\iy} x^{s-1} y^{-s} \, ds \, \gh(dy) \notag \\
         %&= \frac1{2\gp i} \int_{c-i\iy}^{c+\iy} x^{s-1} \int_0^\iy y^{-s} \, \gh(dy) \, ds \notag \\
         &= \frac1{2\gp i} \int_{c-i\iy}^{c+\iy}  x^{s-1} \gzh(s) \, ds, \\
  \noalign{and}
  \gzh(s) &= \int_0^\iy x^{-s} \, \gh(dx).
  \label{eqn:Dirichlet integral}
\end{align}

\begin{defn}
  \label{defn:scaling and geom meas}
  The \emph{scaling measure} encodes all products of scaling ratios
  and is given by
  \begin{align}
    \label{def:scaling measure}
    \ghs(x) := \sum_{w \in W} \gd_{1/r_w}(x).
  \end{align}
  From this, we get the \emph{geometric measure}
  \begin{align}
    \label{def:geom measure}
    \ghg(x) := \sum_{\gr} \gd_{1/\gr}(x)
      &= \sum_{q=1}^Q \sum_{w \in W} \gd_{1/g_q r_w}(x)
      %&= \sum_{q=1}^Q \sum_{w \in W} \gd_{1/r_w} (g_qx) \\
      = \sum_{q=1}^Q \ghs(x/g_q),
  \end{align}
  a sum of horizontally dilated (or ``predilated'') scaling measures.
  In particular, this decomposition exposes the term corresponding to
  each $G_q$; the \emph{\nth[q] geometric measure} is defined
  \(\ghgq(x) := \ghs(x/g_q)\).
\end{defn}

\begin{defn}
  \label{defn:scaling and geom zetas}
  Correspondingly, we also have the \emph{scaling zeta function}
  $\gzs: \bC \to \bC$ which encodes the contributions of all
  generators to the density of geometric states and is given by
  \begin{align}
    \label{def:scaling zeta}
    \gzs(s)
      := \sum_\gr \gr^s
       = \sum_{n=1}^\iy \sum_{j_1=1}^J \dots \sum_{j_n=1}^J
        \left(r_{j_1} \dots r_{j_n}\right)^s
       = \frac1{1-\sum_{j=1}^J r_j^s},
  \end{align}
  and the \emph{geometric zeta function}
  \begin{align}
    \label{def:geom zeta}
    \gzg(s) := \frac{\sum_{q=1}^Q g_q^s}{1-\sum_{j=1}^J r_j^s}
      = \sum_{q=1}^Q g_q^s \gzs(s)
      = \ggh(s) \gzs(s),
  \end{align}
  where $\ggh(s) := \sum_{q=1}^Q g_q^s$. Thus, the geometric zeta
  \fn is a sum of vertically dilated zeta \fns. This decomposition reveals
  the \emph{\nth[q] geometric zeta function} $\gzgq(s):=g_q^s
  \gzs(s)$.
\end{defn}

Note that the equality at the far right side of \eqref{def:scaling
zeta} comes from an application of the geometric series formula
and is consequently only valid for $\Re(s) >D$, where $D$ is as
defined in Def.~\ref{def:complex dimensions}. Examples of these
measures and zeta \fns are given in \S\ref{sec:examples}.

\begin{remark}
  \label{rem:poles and zeros of zeta}
  It is apparent that the poles and zeros of the function $\gzg(s)$
  are
  \begin{align}
    \label{eqn:poles and zeros of zeta}
    \D &\ci \{\text{solutions of } r_1^\gw + \dots r_J^\gw = 1\}
       = \{\text{roots of } 1-\gzs\}, \text{ and} \\
    \Z &\ci \{\text{solutions of } g_1^\gw + \dots g_Q^\gw = 0\}
       = \{\text{roots of } \ggh\}.
  \end{align}
  Note that the poles of \gzg form a subset of the poles of \gzs, as
  roots of \ggh may cancel roots of $1-\gzs$, etc. Clearly,
  cancellation cannot occur in the case of one generator.
\end{remark}

\pgap

\begin{defn}
  \label{def:complex dimensions}
  Following \cite{FGNT}, we define the \emph{complex dimensions}
  of $F$ to be
  \begin{equation*}
    \D := \{\text{poles of \gzg}\}.
  \end{equation*}
  We also single out a particularly important complex dimension
  $D \in \bR$ which is defined by
  $\sum_{j=1}^J r_j^D = 1$.
  The following proposition shows this definition to be valid.
\end{defn}

\begin{prop}
  $D$ is the only real pole of \gzs.
  \begin{proof}
    Consider the \cn \fn
    \begin{equation}
      \label{eqn:real-valued zeta}
      f(s) = \sum_{j=1}^J r_j^s
    \end{equation}
    for \emph{real} values of $s$. Since $0<r_j<1$, $f$ is strictly
    decreasing. Since $f(0) = J > 1$,
    there is a unique value $D > 0$ \st $f(D)=1$.
    \begin{comment}
      We just saw that \gzF has a unique pole in $(0,d)$, and it
      is clear that, as $f$ is a decreasing \fn, \gzF will have no
      other poles on the real line.
    \end{comment}
  \end{proof}
\end{prop}
Note: if we impose a the stronger condition on the $\simt_j$ that
$\sum r_j < 1$, then one can show $0 < D < d$.

\begin{comment}
  As a side note, here is what would happen if you took the areas
  instead of the diameters:
  \begin{align*}
    \tilde{\gz}_{F}(s) &= \sum_{j=1}^\iy \sum_{k=1}^{k_j} m(\tileset_j_k)^s \\
      &= \sum_{n=1}^\iy A_n^s.
  \end{align*}
\end{comment}

\begin{comment}
\begin{remark}
  Possible advantage of this method:
  \begin{enumerate}
    \item There may be some way to extract the spacing information.
      Strings with gaps can be thought of as being spaced by
      another string (as I looked at previously) or as being
      formed by the removal of extra bits during the process
      outlined in [La-vF, 2nd ed.]. However, neither of these
      approaches seems particularly natural. If the components of a
      fractal are spaced in this setting, is is due entirely to
      the IFS $\{\simt_j\}$. Thus, that information can surely be
      recovered from the IFS itself.
    \item Perhaps this can be extended to Kigami's more general
      setting of self-similar structures, some additional conditions
      may be required. The only notion I introduced which is not
      part of a self-similar structure is Lebesgue measure.
  \end{enumerate}
\end{remark}
\end{comment}

\pgap

